Towards Flexible Device Participation in Federated Learning

Traditional federated learning algorithms impose strict requirements on the participation rates of devices, which limit the potential reach of federated learning. This paper extends the current learning paradigm to include devices that may become inactive, compute incomplete updates, and depart or arrive in the middle of training. We derive analytical results to illustrate how allowing more flexible device participation can affect the learning convergence when data is not independently and identically distributed (non-IID). We then propose a new federated aggregation scheme that converges even when devices may be inactive or return incomplete updates. We also study how the learning process can adapt to early departures or late arrivals, and analyze their impacts on the convergence.

==> proof.tex <==
% (The analysis will give a convergence bound for adapting aggregation weights $p_\tau^k$, from which results with fixed weights can be presented as corollaries.)

\section{Algorithm Analysis}

\subsection{Algorithm Description}

Suppose there are $N$ clients, each client $k$ has a local objective $F_k(w)$. The global objective is to minimize $F(w) = \sum_{k=1}^N p^k F_k(w)$, where $p^k = \frac{n_k}{n}$, $n_k$ is the number of data points client $k$ owns and $n = \sum_{k=1}^N n_k$. We bound the non-iid as $\Gamma_k = F_k(w^*) - F_k^*, \Gamma = \sum_{k=1}^N p^k\Gamma_k$.

We consider discrete time steps $t=0,1,\dots,T$. Model weights are synchronized when $t$ is a multiple of $E$ (i.e., the coordinator will do an aggregation every $E$ local rounds). For each global round (say the $\tau$th round), the following three steps are executed:

\begin{itemize}[leftmargin=*]
    \item First, the coordinator broadcasts the latest global weight $w_{\tau E}^{g}$ to all clients. Each client set its local weight $w_{\tau E}^k = w_{\tau E}^{g}$
    \item Second, each client runs SGD on its local objective $F_k$ for $i=0,\dots,s_\tau^k-1$,
    \begin{equation} \label{eq:local_sgd_raw}
        w_{\tau E + i + 1}^k = w_{\tau E + i}^k - \eta_{\tau} g_{\tau E +i}^k
    \end{equation}
    here $\eta_\tau$ is the learning rate that decays over time, $s_\tau^k \leq E$ is a random variable representing the number of local updates this client does in this round, $g_{t}^k = \nabla F_k (w_{t}^k, \xi_{t}^k)$ is the stochastic gradient, and $\xi_{t}^k$ is a mini-batch sampled from client $k$'s local dataset. We also define $\bar{g}_{t}^k = \nabla F_k(w_t^k)$ as the full batch gradient, hence $\bar{g}_t^k = \mathbb{E}_{\xi_t^k}[g_t^k]$.
    \item Third, the coordinator aggregates the next global weight as
    \begin{equation} \label{eq:aggregation_raw}
        w_{(\tau+1)E}^g = w_{\tau E}^g + \sum_{k=1}^N p_\tau^k (w_{\tau E + s_\tau^k} - w_{\tau E}^g) = w_{\tau E}^g - \sum_{k=1}^N p_\tau^k \sum_{i=0}^{s_\tau^k} \eta_{\tau}g_{\tau E + i}^k
    \end{equation}
\end{itemize}

\subsection{Equivalent View}
For ease of the analysis, we introduce for each client $k$ and each global round $\tau$ a sequence of virtual variables $\alpha_{\tau E}^k, \alpha_{\tau E + 1}^k, \dots, \alpha_{(\tau+1)E - 1}^k$. Here each $\alpha_t^k \in \{0,1\}$ and $\sum_{i=0}^E \alpha_{\tau E + i}^k = s_\tau^k$. If $s_\tau^k$ is a random variable, then $\alpha_t^k$'s are also random variables, and the distributions of $\alpha_t^k$'s determine the distribution of $s_\tau^k$. For example, if $\alpha_t^k \overset{iid}{\sim} \textrm{Bernoulli}(p)$, then $s_\tau^k \sim \textrm{Bin}(E,p)$. In this paper, we do not make any assumption on the distributions and correlations of $\alpha_t^k$'s. Our results are thus valid for any realization of $s_\tau^k$. 
% For convenience, we write ${g_t^k}' = g_t^k \alpha_t^k$

With the definition of $\alpha_t^k$'s, we can rewrite (\ref{eq:local_sgd_raw})(\ref{eq:aggregation_raw}) as:

\begin{equation} \label{eq:local_sgd}
    w_{\tau E + i + 1}^k = w_{\tau E + i}^k - \eta_{\tau} g_{\tau E +i}^k\alpha_{\tau E + i}^k
\end{equation}

\begin{equation} \label{eq:aggregation}
    w_{(\tau+1)E}^g = w_{\tau E}^g - \sum_{k=1}^N p_\tau^k \sum_{i=0}^{E} \eta_{\tau}g_{\tau E + i}^k\alpha_{\tau E + i}^k
\end{equation}

Note that $w_t^g$ is visible only when $t$ is a multiple of $E$. To generalize it to arbitrary $t$, we define $\bar{w}_t$ such that $\bar{w}_0 = w_0^g$, and
\begin{equation}\label{eq:w_bar}
\bar{w}_{\tau E + i + 1} = \bar{w}_{\tau E + i} - \eta_{\tau}\sum_{k=1}^N p_\tau^k g_{\tau E + i}^k \alpha_{\tau E + i}
\end{equation}
Note that $\bar{w}_{\tau E + i} = \sum_{k=1}^N p_\tau^k w_{\tau E + i}^k$ only if $\sum_{k=1}^N p_\tau^k = 1$, which generally does not hold.


\begin{lemma}
For any $\tau$, $\bar{w}_{\tau E} = w_{\tau E}^g$.
\end{lemma}

\begin{proof}
We will prove by induction. By definition, $\bar{w}_0 = w_0^g$. Suppose $\bar{w}_{\tau E} = w_{\tau E}^g$, then
\begin{equation}
\begin{split}
    \bar{w}_{(\tau+1) E} &= \bar{w}_{(\tau+1) E - 1} - \eta_{\tau}\sum_{k=1}^N p_\tau^k g_{(\tau+1) E - 1}^k \alpha_{(\tau+1) E - 1} \\
    &= \dots = \bar{w}_{\tau E} - \sum_{i=0}^{E-1}\eta_{\tau}\sum_{k=1}^N p_\tau^k g_{\tau E + i}^k \alpha_{\tau E + i}\\
    &= w_{\tau E}^g - \sum_{k=1}^N p_\tau^k \sum_{i=0}^{E-1} \eta_{\tau}g_{\tau E + i}^k\alpha_{\tau E + i}^k = w_{(\tau + 1)E}^g
\end{split}
\end{equation}
\end{proof}

Thus, in the following analysis we will just use $\bar{w}_t$ to denote the global weight.

\subsection{Assumptions}
The analysis relies on the following assumptions:
\begin{assumption} \label{asm:Lsmooth}
$F_1,\dots,F_N$ are all $L$-smooth.
\end{assumption}
\begin{assumption} \label{asm:mu_strong}
$F_1,\dots,F_N$ are all $\mu$-strongly convex.
\end{assumption}
\begin{assumption} \label{asm:sigma2}
The variance of stochastic gradients in each device is bounded: $\mathbb{E}_{\xi} \Vert g_t^k - \bar{g}_t^k \Vert^2 \leq \sigma_k^2$ for all $k$ and $t$.
\end{assumption}
\begin{assumption} \label{asm:G2}
The expected squared norm of stochastic gradients is uniformly bounded: $\mathbb{E}_\xi \Vert g_t^k \Vert^2 \leq G^2$ for all $k$ and $t$.
\end{assumption}
\begin{assumption} \label{asm:cp}
There exists an upper bound $\frac{p_\tau^k}{p^k} \leq c_p$
\end{assumption}

\section{Convergence Rate}
We first present a couple of important lemmas:

\begin{lemma} \label{lm:grad_var}
\begin{equation}
    \mathbb{E}_\xi \Vert \sum_{k=1}^N p_\tau^k (g_t^k - \bar{g}_t^k) \Vert^2 \leq \sum_{k=1}^N (p_\tau^k)^2 \sigma_k^2
\end{equation}
\end{lemma}

\begin{proof}
\begin{equation}
    \Vert \sum_{k=1}^N p_\tau^k (g_t^k - \bar{g}_t^k) \Vert^2 = \sum_{k=1}^N \Vert p_\tau^k (g_t^k - \bar{g}_t^k) \Vert^2 + \sum_{j\neq k} \Vert p_\tau^k p_\tau^j (g_t^k - \bar{g}_t^k)(g_t^j - \bar{g}_t^j) \Vert^2
\end{equation}
Since each client is running independently, the covariance
\begin{equation}
    \mathbb{E}_\xi \Vert (g_t^k - \bar{g}_t^k)(g_t^j - \bar{g}_t^j) \Vert^2 = 0
\end{equation}
Thus,
\begin{equation}
    \mathbb{E}_\xi \Vert \sum_{k=1}^N p_\tau^k (g_t^k - \bar{g}_t^k) \Vert^2 = \sum_{k=1}^N \mathbb{E}_\xi \Vert p_\tau^k (g_t^k - \bar{g}_t^k) \Vert^2 \leq \sum_{k=1}^N (p_\tau^k)^2 \sigma_k^2
\end{equation}
\end{proof}

\begin{lemma} \label{lm:local_global_div}
\begin{equation}
    \mathbb{E}_\xi [\sum_{k=1}^N p_\tau^k \Vert \bar{w}_{\tau E + i} - w_{\tau E + i}^k \Vert^2] \leq (E-1)G^2\eta_\tau^2\Big(\sum_{k=1}^Np_\tau^k s_\tau^k + (\sum_{k=1}^N p_\tau^k - 2)_+\sum_{k=1}^N \frac{(p_\tau^k)^2}{p^k}s_\tau^k \Big)
\end{equation}
\end{lemma}

\begin{proof}
Note that $w_{\tau E}^k = \bar{w}_{\tau E}$ for all $k$.
\begin{equation}
\begin{split}
    \Vert \bar{w}_{\tau E + i} &- w_{\tau E + i}^k \Vert^2 = \Vert (\bar{w}_{\tau E + i} - \bar{w}_{\tau E}) - (w_{\tau E + i}^k - \bar{w}_{\tau E}) \Vert^2 \\
    &= \Vert \bar{w}_{\tau E + i} - \bar{w}_{\tau E} \Vert^2 - 2 \langle \bar{w}_{\tau E + i} - \bar{w}_{\tau E}, w_{\tau E + i}^k - \bar{w}_{\tau E} \rangle + \Vert w_{\tau E + i}^k - \bar{w}_{\tau E} \Vert^2
\end{split}
\end{equation}
From (\ref{eq:local_sgd})(\ref{eq:w_bar}),

\begin{equation}
\begin{split}
        \sum_{k=1}^N p_\tau^k w_{\tau E + i}^k &= \sum_{k=1}^N p_\tau^k w_{\tau E + i -1}^k - \eta_{\tau}\sum_{k=1}^N p_\tau^k g_{\tau E + i - 1}^k\alpha_{\tau E + i - 1}^k \\
        &= \sum_{k=1}^N p_\tau^k w_{\tau E + i -1}^k + \bar{w}_{\tau E + i} - \bar{w}_{\tau E + i - 1}\\
        &= \dots = \sum_{k=1}^N p_\tau^k w_{\tau E}^k + \bar{w}_{\tau E + i} - \bar{w}_{\tau E}
\end{split}
\end{equation}
Thus,
\begin{equation}
\begin{split}
        &- 2 \sum_{k=1}^N p_\tau^k \langle \bar{w}_{\tau E + i} - \bar{w}_{\tau E}, w_{\tau E + i}^k - \bar{w}_{\tau E} \rangle \\
        =& - 2  \langle \bar{w}_{\tau E + i} - \bar{w}_{\tau E}, \sum_{k=1}^N p_\tau^k w_{\tau E}^k + \bar{w}_{\tau E + i} - \bar{w}_{\tau E} - \sum_{k=1}^N p_\tau^k \bar{w}_{\tau E} \rangle\\
        =& -2 \Vert \bar{w}_{\tau E + i} - \bar{w}_{\tau E} \Vert^2
\end{split}
\end{equation}

\begin{equation}\label{eq:lemma2_0}
    \sum_{k=1}^N p_\tau^k \Vert \bar{w}_{\tau E + i} - w_{\tau E + i}^k \Vert^2 = (\sum_{k=1}^N p_\tau^k - 2) \Vert \bar{w}_{\tau E + i} - \bar{w}_{\tau E} \Vert^2 + \sum_{k=1}^N p_\tau^k \Vert w_{\tau E + i}^k - \bar{w}_{\tau E} \Vert^2
\end{equation}

\begin{equation} \label{eq:lemma2_1}
\begin{split}
    &\Vert \bar{w}_{\tau E + i} - \bar{w}_{\tau E} \Vert^2 = \Vert \sum_{j=0}^{i-1} \eta_\tau \sum_{k=1}^N p_\tau^k g_{\tau E + j}^k \alpha_{\tau E + j}^k \Vert^2 \\
    =& \Vert \eta_\tau \sum_{k=1}^N p_\tau^k \Big(\sum_{j=0}^{i-1} g_{\tau E + j}^k \alpha_{\tau E + j}^k\Big) \Vert^2 = \eta_\tau^2 \Vert \sum_{k=1}^N p^k \Big( \frac{p_\tau^k}{p^k} \sum_{j=0}^{i-1} g_{\tau E + j}^k \alpha_{\tau E + j}^k\Big) \Vert^2\\
    \leq &\eta_\tau^2 \sum_{k=1}^N \frac{(p_\tau^k)^2}{p^k} \Vert \sum_{j=0}^{i-1} g_{\tau E + j}^k \alpha_{\tau E + j}^k \Vert^2
\end{split}
\end{equation}

Here
\begin{equation}
\begin{split}
        \Vert \sum_{j=0}^{i-1} g_{\tau E + j}^k \alpha_{\tau E + j}^k \Vert^2 &= \sum_{j=0}^{i-1} \Vert g_{\tau E + j}^k\alpha_{\tau E + j}^k \Vert^2 + 2\sum_{p < q} \langle g_{\tau E + p}^k \alpha_{\tau E + p}^k,g_{\tau E + q}^k \alpha_{\tau E + q}^k \rangle \\
        &\leq \sum_{j=0}^{i-1} \Vert g_{\tau E + j}^k\alpha_{\tau E + j}^k \Vert^2 + 2\sum_{p< q} \Vert g_{\tau E + p}^k \alpha_{\tau E + p}^k \Vert \Vert g_{\tau E + q}^k \alpha_{\tau E + q}^k \Vert \\
        &\leq \sum_{j=0}^{i-1} \Vert g_{\tau E + j}^k\alpha_{\tau E + j}^k \Vert^2 + \sum_{p < q}\Big(\Vert g_{\tau E + p}^k \alpha_{\tau E + p}^k \Vert + \Vert g_{\tau E + q}^k \alpha_{\tau E + q}^k \Vert \Big) \\
        &= i\sum_{j=0}^{i-1}\Vert g_{\tau E + j}^k\alpha_{\tau E + j}^k \Vert^2
\end{split}
\end{equation}

So
\begin{equation} \label{eq:lemma2_2}
    \mathbb{E}_{\xi} \Vert \sum_{j=0}^{i-1} g_{\tau E + j}^k \alpha_{\tau E + j}^k \Vert^2 \leq iG^2 \sum_{j=0}^{i-1} \alpha_{\tau E + j}^k \leq (E-1)G^2s_\tau^k
\end{equation}

Plug (\ref{eq:lemma2_2}) to (\ref{eq:lemma2_1}) we have
\begin{equation} \label{eq:lemma2_3}
\begin{split}
        \mathbb{E}_{\xi} \Vert \bar{w}_{\tau E + i} - \bar{w}_{\tau E} \Vert^2 \leq (E-1)G^2\eta_\tau^2\sum_{k=1}^N \frac{(p_\tau^k)^2}{p^k} s_\tau^k
\end{split}
\end{equation}

Similarly
\begin{equation} \label{eq:lemma2_4}
\begin{split}
    \mathbb{E}_\xi\sum_{k=1}^N p_\tau^k \Vert w_{\tau E + i}^k - \bar{w}_{\tau E} \Vert^2 = \mathbb{E}_\xi\sum_{k=1}^N p_\tau^k \Vert \eta_\tau \sum_{j=0}^{i-1} g_{\tau E + j}^k \alpha_{\tau E + j}^k \Vert^2 \leq (E-1)G^2\eta_\tau^2 \sum_{k=1}^N p_\tau^k s_\tau^k
\end{split}
\end{equation}

Plug (\ref{eq:lemma2_3})(\ref{eq:lemma2_4}) to (\ref{eq:lemma2_0}) we have
\begin{equation}
    \mathbb{E}_\xi [\sum_{k=1}^N p_\tau^k \Vert \bar{w}_{\tau E + i} - w_{\tau E + i}^k \Vert^2] \leq (E-1)G^2\eta_\tau^2\Big(\sum_{k=1}^Np_\tau^k s_\tau^k + (\sum_{k=1}^N p_\tau^k - 2)_+\sum_{k=1}^N \frac{(p_\tau^k)^2}{p^k}s_\tau^k \Big)
\end{equation}
\end{proof}

\subsection{Bounding $\Vert \bar{w}_{\tau E + i + 1} - w^* \Vert^2$}
\begin{equation} \label{eq:|w_bar-w*|}
\begin{split}
    \Vert \bar{w}_{\tau E + i + 1} - w^* \Vert^2 &= \Vert\bar{w}_{\tau E + i} - \eta_\tau \sum_{k=1}^N p_\tau^k \alpha_{\tau E + i}^k g_{\tau E + i}^k - w^* - \eta_{\tau} \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k \bar{g}_{\tau E + i}^k + \eta_{\tau} \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k \bar{g}_{\tau E + i}^k \Vert^2 \\
    &= \underbrace{\Vert\bar{w}_{\tau E + i} - w^* - \eta_{\tau} \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k \bar{g}_{\tau E + i}^k\Vert^2}_{A_1} + \eta_\tau^2 \Vert \sum_{k=1}^Np_\tau^k\alpha_{\tau E + i}^k(\bar{g}_{\tau E + i}^k - g_{\tau E + i}^k) \Vert^2 \\
    &+ \underbrace{2\eta_\tau \langle \bar{w}_{\tau E + i} - w^* - \eta_{\tau} \sum_{k=1}^Np_\tau^k\alpha_{\tau E + i}^k\bar{g}_{\tau E + i}^k, \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k (\bar{g}_{\tau E + i}^k - g_{\tau E + i}^k) \rangle}_{A_2}
\end{split}
\end{equation}

Since $\mathbb{E}_\xi [g_{\tau E + i}^k] = \bar{g}_{\tau E + i}^k$, we have $\mathbb{E}_{\xi} [A_2] = 0$. We then bound $A_1$.
\begin{equation} \label{eq:A1_0}
\begin{split}
        &A_1 = \Vert\bar{w}_{\tau E + i} - w^* - \eta_{\tau} \sum_{k=1}^N p_\tau^k \alpha_{\tau E + i}^k \bar{g}_{\tau E + i}^k\Vert^2\\
        =& \Vert \bar{w}_{\tau E + i} - w^* \Vert^2 \underbrace{- 2\eta_t \langle \bar{w}_{\tau E + i} - w^*, \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k \bar{g}_{\tau E + i}^k \rangle}_{B_1} + \underbrace{\eta_t^2 \Vert \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k \bar{g}_{\tau E + i}^k \Vert^2}_{B_2}
\end{split}
\end{equation}

Since $F_k$ is $L$-smooth,
\begin{equation}
    \Vert \alpha_{\tau E + i}^k\bar{g}_{\tau E + i}^k \Vert^2 \leq 2L (F_k(w_{\tau E + i}^k) - F_k^*)\alpha_{\tau E + i}^k
\end{equation}

By the convexity of $l_2$ norm
\begin{equation} \label{eq:B2}
\begin{split}
        B_2 &= \eta_\tau^2 \Vert \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k \bar{g}_{\tau E + i}^k \Vert^2 = \eta_\tau^2\Vert \sum_{k=1}^N p^k (\frac{p_\tau^k}{p^k}\alpha_{\tau E + i}^k \bar{g}_{\tau E + i}^k) \Vert^2\\
        &\leq \eta_\tau^2 \sum_{k=1}^N \frac{(p_\tau^k)^2}{p^k} \Vert \alpha_{\tau E + i}^k\bar{g}_{\tau E + i}^k \Vert^2 \leq 2Lc_p\eta_\tau^2 \sum_{k=1}^N p_\tau^k (F_k(w_{\tau E + i}^k) - F_k^*) \alpha_{\tau E + i}^k
\end{split}
\end{equation}

\begin{equation} \label{eq:B1}
\begin{split}
    B_1 &= - 2\eta_\tau \langle \bar{w}_{\tau E + i} - w^*, \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k \bar{g}_{\tau E + i}^k \rangle = -2\eta_\tau \sum_{k=1}^N p_\tau^k \langle \bar{w}_{\tau E + i} - w^*, \alpha_{\tau E + i}^k \bar{g}_{\tau E + i}^k \rangle \\
    &= -2\eta_\tau \sum_{k=1}^N p_\tau^k \langle \bar{w}_{\tau E + i} - w_{\tau E + i}^k, \alpha_{\tau E + i}^k \bar{g}_{\tau E + i}^k \rangle - 2\eta_\tau \sum_{k=1}^N p_k \langle w_{\tau E + i}^k -w^*, \alpha_{\tau E + i}^k \bar{g}_{\tau E + i}^k\rangle
\end{split}
\end{equation}
Here
\begin{equation} \label{eq:B1_1}
\begin{split}
    &-2\langle\bar{w}_{\tau E + i} - w_{\tau E + i}^k, \alpha_{\tau E + i}^k \bar{g}_{\tau E + i}^k \rangle \leq 2 |\langle \bar{w}_{\tau E + i} - w_{\tau E + i}^k, \alpha_{\tau E + i}^k \bar{g}_{\tau E + i}^k \rangle| \\
    \leq& 2 \alpha_{\tau E + i}^k\Vert \bar{w}_{\tau E + i} - w_{\tau E + i}^k\Vert \Vert \bar{g}_{\tau E + i}^k\Vert \leq \Big(\frac{1}{\eta_\tau} \Vert \bar{w}_{\tau E + i} - w_{\tau E + i}^k \Vert^2 + \eta_\tau \Vert \bar{g}_{\tau E + i}^k \Vert^2\Big)\alpha_{\tau E + i}^k
\end{split}
\end{equation}
Since $F_k$ is $\mu$-strong convex
\begin{equation} \label{eq:B1_2}
    \langle w_{\tau E + i}^k - w^*, \alpha_{\tau E + i}^k\bar{g}_{\tau E + i}^k \rangle \geq \big((F_k(w_{\tau E + i}^k) - F_k(w^*)) + \frac{\mu}{2} \Vert w_{\tau E + i}^k - w^* \Vert^2\big)\alpha_{\tau E + i}^k
\end{equation}

Plug (\ref{eq:B1_1})(\ref{eq:B1_2}) to (\ref{eq:B1})
\begin{equation} \label{eq:B1_final}
\begin{split}
        B_1 \leq  \sum_{k=1}^N p_\tau^k \alpha_{\tau E + i}^k \Bigg(\Vert \bar{w}_{\tau E + i} - w_{\tau E + i}^k \Vert^2 + \eta_\tau^2 \Vert \bar{g}_{\tau E + i}^k \Vert^2 - 2\eta_\tau \big((F_k(w_{\tau E + i}^k) - F_k(w^*)) + \frac{\mu}{2} \Vert w_{\tau E + i}^k - w^* \Vert^2\big) \Bigg)
\end{split}
\end{equation}

Plug (\ref{eq:B2})(\ref{eq:B1_final}) to (\ref{eq:A1_0})
\begin{equation}
\begin{split}
    A_1 &\leq \Vert\bar{w}_{\tau E + i} - w^* \Vert^2 + 2Lc_p\eta_\tau^2 \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k (F_k(w_{\tau E + i}^k) - F_k^*) \\
    &+ \sum_{k=1}^N p_\tau^k \alpha_{\tau E + i}^k \Bigg(\Vert \bar{w}_{\tau E + i} - w_{\tau E + i}^k \Vert^2 + \underbrace{\eta_\tau^2 \Vert \bar{g}_{\tau E + i}^k \Vert^2}_{\leq  2\eta_\tau^2 L(F_k(w_{\tau E + i}^k) - F_k^*)} - 2\eta_\tau \big((F_k(w_{\tau E + i}^k) - F_k(w^*)) + \frac{\mu}{2} \Vert w_{\tau E + i}^k - w^* \Vert^2\big) \Bigg) \\
    &\leq \Vert \bar{w}_{\tau E + i} - w^* \Vert^2 - \mu\eta_\tau\sum_{k=1}^N p_\tau^k \alpha_{\tau E + i}^k \Vert w_{\tau E + i}^k - w^* \Vert^2 + \sum_{k=1}^N p_\tau^k \alpha_{\tau E + i}^k \Vert \bar{w}_{\tau E + i} - w_{\tau E + i}^k \Vert^2\\
    &+\underbrace{2(1+c_p)L\eta_\tau^2\sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k (F_k(w_{\tau E + i}^k) - F_k^*) - 2\eta_\tau \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k (F_k(w_{\tau E + i}^k) - F_k(w^*))}_{C}
\end{split}
\end{equation}

\begin{equation}
\begin{split}
        \Vert w_{\tau E + i}^k - w^* \Vert^2 &= \Vert w_{\tau E + i}^k - \bar{w}_{\tau E + i} + \bar{w}_{\tau E + i} - w^* \Vert^2 \\
        &= \Vert w_{\tau E + i}^k - \bar{w}_{\tau E + i} \Vert^2 + \Vert \bar{w}_{\tau E + i} - w^* \Vert^2 + 2\langle w_{\tau E + i}^k-\bar{w}_{\tau E + i},\bar{w}_{\tau E + i}-w^*\rangle \\
        &\geq \Vert w_{\tau E + i}^k - \bar{w}_{\tau E + i} \Vert^2 + \Vert \bar{w}_{\tau E + i} - w^* \Vert^2 - 2\Vert w_{\tau E + i}^k-\bar{w}_{\tau E + i}\Vert \Vert\bar{w}_{\tau E + i} - w^* \Vert \\
        &\geq \Vert w_{\tau E + i}^k - \bar{w}_{\tau E + i} \Vert^2 + \Vert \bar{w}_{\tau E + i} - w^* \Vert^2 - (2\Vert w_{\tau E + i}^k-\bar{w}_{\tau E + i}\Vert^2 + \frac{1}{2} \Vert\bar{w}_{\tau E + i} - w^* \Vert^2)\\
        &= \frac{1}{2} \Vert\bar{w}_{\tau E + i} - w^* \Vert^2 - \Vert w_{\tau E + i}^k - \bar{w}_{\tau E + i} \Vert^2
\end{split}
\end{equation}
Thus,
\begin{equation} \label{eq:A1}
    A_1 \leq (1-\frac{1}{2}\mu\eta_\tau\sum_{k=1}^N p_\tau^k \alpha_{\tau E + i}^k) \Vert \bar{w}_{\tau E + i} - w^* \Vert^2 + (1+\mu \eta_\tau)\sum_{k=1}^N p_\tau^k \alpha_{\tau E + i}^k \Vert \bar{w}_{\tau E + i} - w_{\tau E + i}^k \Vert^2 + C
\end{equation}

Let $\gamma_\tau = 2\eta_\tau(1-(1+c_p)L\eta_\tau)$. Assume $\eta_\tau \leq \frac{1}{2(1+c_p)L}$, hence $\eta_\tau \leq \gamma_\tau \leq 2\eta_\tau$.
\begin{equation}
\begin{split}
    C &= -2\eta_\tau(1-(1+c_p)L\eta_\tau)\sum_{k=1}^Np_\tau^k\alpha_{\tau E + i}^k(F_k(w_{\tau E + i}^k)-F_k^*) + 2\eta_\tau\sum_{k=1}^Np_\tau^k\alpha_{\tau E + i}^k(F_k(w^*)-F_k^*)\\
    &= -\gamma_\tau \sum_{k=1}^Np_\tau^k\alpha_{\tau E + i}^k (F_k(w_{\tau E + i}^k)- F_k^* + F_k(w^*)-F_k(w^*)) + 2\eta_\tau\sum_{k=1}^Np_\tau^k\alpha_{\tau E + i}^k(F_k(w^*)-F_k^*)\\
    &= -\gamma_\tau \sum_{k=1}^Np_\tau^k\alpha_{\tau E + i}^k (F_k(w_{\tau E + i}^k)-F_k(w^*)) + (2\eta_\tau-\gamma_\tau)\sum_{k=1}^Np_\tau^k\alpha_{\tau E + i}^k(F_k(w^*)-F_k^*)\\
    &\leq \underbrace{-\gamma_\tau \sum_{k=1}^Np_\tau^k\alpha_{\tau E + i}^k (F_k(w_{\tau E + i}^k)-F_k(w^*))}_{D} + 2(1+c_p)L\eta_\tau^2\sum_{k=1}^Np_\tau^k\alpha_{\tau E + i}^k\Gamma_k\\
\end{split}
\end{equation}

Next we bound $D$
\begin{equation}
\begin{split}
    &\sum_{k=1}^Np_\tau^k\alpha_{\tau E + i}^k (F_k(w_{\tau E + i}^k)- F_k(w^*)) = \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k ( F_k(w_{\tau E + i}^k) - F_k(\bar{w}_{\tau E + i})) + \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k (F_k(\bar{w}_{\tau E + i})-F_k(w^*)) \\
    &\geq \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k \langle \nabla F_k(\bar{w}_{\tau E + i}), w_{\tau E + i}^k - \bar{w}_{\tau E + i} \rangle + \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k (F_k(\bar{w}_{\tau E + i})-F_k(w^*)) \\
    &\geq -\sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k  \Vert \nabla F_k(\bar{w}_{\tau E + i}) \Vert \Vert w_{\tau E + i}^k - \bar{w}_{\tau E + i}\Vert + \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k (F_k(\bar{w}_{\tau E + i})-F_k(w^*)) \\
    &\geq - \frac{1}{2}\sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k  (\eta_\tau \underbrace{\Vert \nabla F_k(\bar{w}_{\tau E + i}) \Vert^2}_{\leq 2L (F_k(\bar{w}_{\tau E + i})-F_k^*)} + \frac{1}{\eta_\tau} \Vert w_{\tau E + i}^k - \bar{w}_{\tau E + i} \Vert^2) + \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k (F_k(\bar{w}_{\tau E + i})-F_k(w^*)) \\
    &\geq - \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k \Big(\eta_\tau L   (F_k(\bar{w}_{\tau E + i}) - F_k^*) + \frac{1}{2\eta_\tau}  \Vert w_{\tau E + i}^k - \bar{w}_{\tau E + i} \Vert^2 \Big) + \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k (F_k(\bar{w}_{\tau E + i})-F_k(w^*))
\end{split}
\end{equation}
Thus,
\begin{equation} \label{eq:C}
\begin{split}
        C &\leq \gamma_\tau\sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k (\eta_\tau L  \underbrace{(F_k(\bar{w}_{\tau E + i})-F_k^*)}_{F_k(\bar{w}_{\tau E + i})-F_k(w^*) + F_k(w^*) - F_k^*}+\frac{1}{2\eta_\tau}\Vert w_{\tau E + i}^k - \bar{w}_{\tau E + i} \Vert^2) \\
        &\;\;\;\;\;\;\;- \gamma_\tau \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k (F_k(\bar{w}_{\tau E + i})-F_k(w^*)) + 2(1+c_p)L\eta_\tau^2 \sum_{k=1}^N p_\tau^k \alpha_{\tau E + i} \Gamma_k \\
        &= \gamma_\tau (\eta_\tau L -1) \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k (F_k(\bar{w}_{\tau E + i}) - F_k(w^*)) + \underbrace{\frac{\gamma_\tau}{2\eta_\tau}}_{\leq 1}\sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k \Vert w_{\tau E + i}^k - \bar{w}_{\tau E + i} \Vert^2\\
        &\;\;\;\;\;\;\;+ 2(1+c_p)L\eta_\tau^2 \sum_{k=1}^N p_\tau^k \alpha_{\tau E + i} \Gamma_k + \underbrace{\gamma_\tau}_{\leq 2\eta_\tau}\eta_\tau L \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k \Gamma_k\\
        &\leq \gamma_\tau (\eta_\tau L -1) \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k (F_k(\bar{w}_{\tau E + i}) - F_k(w^*)) + \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k \Vert w_{\tau E + i}^k - \bar{w}_{\tau E + i} \Vert^2\\
        &\;\;\;\;\;\;\; + 2(2+c_p)L\eta_\tau^2 \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k \Gamma_k
\end{split}
\end{equation}

Plug (\ref{eq:C}) to (\ref{eq:A1}) we have
\begin{equation} \label{eq:A1_final}
\begin{split}
        A_1 &\leq \Vert \bar{w}_{\tau E + i} - w^* \Vert^2 - \mu\eta_\tau\sum_{k=1}^N p_\tau^k \alpha_{\tau E + i}^k \Vert w_{\tau E + i}^k - w^* \Vert^2 + 2\sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k \Vert \bar{w}_{\tau E + i} - w_{\tau E + i}^k \Vert^2 \\
        & + 2(2+c_p)L\eta_\tau^2 \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k \Gamma_k + \gamma_\tau (\eta_\tau L -1) \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k (F_k(\bar{w}_{\tau E + i}) - F_k(w^*))
\end{split}
\end{equation}

Plug (\ref{eq:A1_final}) to (\ref{eq:|w_bar-w*|}), 
\begin{equation} \label{eq:recursion0}
\begin{split}
    &\Vert \bar{w}_{\tau E + i + 1} - w^* \Vert^2 \leq (1-\frac{1}{2}\mu\eta_\tau\sum_{k=1}^N p_\tau^k \alpha_{\tau E + i}^k) \Vert \bar{w}_{\tau E + i} - w^* \Vert^2 \\
    +&\eta_\tau^2 \Vert \sum_{k=1}^Np_\tau^k\alpha_{\tau E + i}^k(\bar{g}_{\tau E + i}^k - g_{\tau E + i}^k) \Vert^2 + \underbrace{(2+\mu\eta_\tau)}_{\leq 2 + \frac{\mu}{2(1+c_p)L}}\sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k \Vert \bar{w}_{\tau E + i} - w_{\tau E + i}^k \Vert^2\\
    +& 2(2+c_p)L\eta_\tau^2 \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k \Gamma_k + \underbrace{\gamma_\tau (1 - \eta_\tau L )}_{\leq 2\eta_\tau} \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k (F_k(w^*) - F_k(\bar{w}_{\tau E + i}))
\end{split}
\end{equation}

Define 
\begin{equation}
\begin{split}
        B_{\tau E + i} = (2 + \frac{\mu}{2(1+c_p)L}) \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k \Vert \bar{w}_{\tau E + i} - w_{\tau E + i}^k \Vert^2 &+ \Vert \sum_{k=1}^Np_\tau^k\alpha_{\tau E + i}^k(\bar{g}_{\tau E + i}^k - g_{\tau E + i}^k) \Vert^2 \\
        &+ 2(2+c_p)L \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k \Gamma_k
\end{split}
\end{equation}

Thus,
\begin{equation} \label{eq:recursion0}
\begin{split}
    &\Vert \bar{w}_{\tau E + i + 1} - w^* \Vert^2 \leq (1-\frac{1}{2}\mu\eta_\tau\sum_{k=1}^N p_\tau^k \alpha_{\tau E + i}^k) \Vert \bar{w}_{\tau E + i} - w^* \Vert^2 + \eta_\tau^2B_{\tau E + i}\\
    +& 2\eta_\tau \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k ( F_k(w^*) - F_k(\bar{w}_{\tau E + i}))
\end{split}
\end{equation}

Apply the lemmas we have

\begin{equation}
\begin{split}
        \mathbb{E}_\xi &[B_{\tau E + i}] \leq \sum_{k=1}^N (p_\tau^k)^2\alpha_{\tau E + i}^k \sigma_k^2  + 2(2+c_p)L \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k \Gamma_k\\
        &+(2 + \frac{\mu}{2(1+c_p)L})(E-1)G^2\Big(\sum_{k=1}^Np_\tau^k s_\tau^k + (\sum_{k=1}^N p_\tau^k - 2)_+\sum_{k=1}^N \frac{(p_\tau^k)^2}{p^k}s_\tau^k \Big)
\end{split}
\end{equation}

For convenience we write $\Delta_{\tau E + i} = \Vert \bar{w}_{\tau E + i} - w^* \Vert^2$, and $\bar{\Delta}_{\tau E + i} = \mathbb{E}[\Delta_{\tau E + i}]$, where the expectation is taken over all random variables up to $\tau E + i$.

% \begin{theorem}
% Suppose $s_\tau^k \overset{iid}{\sim} \textrm{Bin}(E,\alpha_\tau)$, then when using $p_\tau^k = p^k$, we have $\bar{\Delta}_{\tau E + i} \leq \frac{v}{(\tau E + i) + \gamma}$, where $\gamma = \frac{16L}{\mu\alpha_0}$, $v =\max \{ \frac{64B_0}{\mu^2(\min_\tau\alpha_\tau)}, \bar{\Delta}_0 \gamma\}$, $B_0 = \sum_{k=1}^N (p^k \sigma_k)^2 + 6L \Gamma + (2+\frac{\mu}{4L})(E-1)EG^2$.

% \end{theorem}

% \begin{proof}
% Let $\alpha_{\tau E + i}^k \overset{iid}{\sim} \textrm{Bernoulli}(\alpha_\tau)$, which satisfies the assumption $s_\tau^k \overset{iid}{\sim} \textrm{Bin}(E,\alpha_\tau)$. Note that $w_{\tau E+ i}^k$ depends on $\alpha_{0}^k,\dots,\alpha_{\tau E + i-1}^k$. Thus, (\ref{eq:recursion0}) can be written as

% \begin{equation}
% \begin{split}
%         &\mathbb{E}_{\boldsymbol{\alpha}_{\tau E + i}|\boldsymbol{\alpha}_{0:\tau E+i-1}}\mathbb{E}_\xi[\Delta_{\tau E + i + 1}] \leq (1-\frac{1}{2}\mu\alpha_\tau\eta_\tau) \mathbb{E}_{\boldsymbol{\alpha}_{\tau E + i}|\boldsymbol{\alpha}_{0:\tau E+i-1}}\mathbb{E}_\xi[\Delta_{\tau E + i}] \\
%         +& \eta_\tau^2 \mathbb{E}_{\boldsymbol{\alpha}_{\tau E + i}|\boldsymbol{\alpha}_{0:\tau E+i-1}}\mathbb{E}_\xi[B_{\tau E + i}]
%         + 2\alpha_\tau\eta_\tau \mathbb{E}_{\boldsymbol{\alpha}_{\tau E + i}|\boldsymbol{\alpha}_{0:\tau E+i-1}}\mathbb{E}_\xi[F(w^*) - F(\bar{w}_{\tau E + i})]
% \end{split}
% \end{equation}

% Here $\mathbb{E}_{\boldsymbol{\alpha}_{\tau E + i}|\boldsymbol{\alpha}_{0:\tau E+i-1}}$ denotes the conditional expectation over $\alpha_{\tau E + i}^1,\dots,\alpha_{\tau E + i}^N$, given $\alpha_{t}^k$ for all $1\leq k \leq N$ and $0 \leq t \leq \tau E + i -1$. 

% When $p_\tau^k = p^k$, $c_p = 1$, thus
% \begin{equation}
% \begin{split}
%         \mathbb{E}_{\boldsymbol{\alpha}_{\tau E + i}|\boldsymbol{\alpha}_{0:\tau E+i-1}}\mathbb{E}_\xi &[B_{\tau E + i}] \leq \alpha_\tau\underbrace{ \sum_{k=1}^N (p^k \sigma_k)^2 + 6L \Gamma + (2+\frac{\mu}{4L})(E-1)EG^2}_{B_{0}}
% \end{split}
% \end{equation}

% We note that $F(w^*) - F(\bar{w}_{\tau E + i}) \leq 0$. With law of iterated expectation we have
% \begin{equation}
% \mathbb{E}_{\boldsymbol{\alpha}_{0:\tau E+i}}\mathbb{E}_\xi[\Delta_{\tau E + i + 1}] \leq (1-\frac{1}{2}\mu\alpha_\tau\eta_\tau) \mathbb{E}_{\boldsymbol{\alpha}_{0:\tau E+i}}\mathbb{E}_\xi[\Delta_{\tau E + i}] + \eta_\tau^2 B_{0}
% \end{equation}

% We then prove the theorem by induction. Initially, $\frac{v}{\gamma} \geq \bar{\Delta}_0$. Suppose $\bar{\Delta}_{\tau E + i} \leq \frac{v}{(\tau E + i) + \gamma}$. Let $\eta_\tau = \frac{4}{\mu \alpha_\tau} \frac{1}{\tau E + \gamma}$, note that $-\frac{1}{\tau E + \gamma} \leq -\frac{1}{\tau E + i + \gamma}$ for all $i \leq E$.

% \begin{equation}
% \begin{split}
%         \bar{\Delta}_{\tau E + i + 1} &\leq (1-\frac{2}{\tau E + \gamma})\bar{\Delta}_{\tau E + i} + \frac{\frac{16\alpha_\tau B_0}{(\mu\alpha_\tau)^2}}{(\tau E + \gamma)^2}\\
%         &\leq (1-\frac{2}{(\tau E + i) + \gamma}) \frac{v}{(\tau E + i) + \gamma}  + \frac{\frac{16\alpha_\tau B_0}{(\mu\alpha_\tau)^2}(\frac{(\tau E + i) + \gamma}{\tau E + \gamma})^2}{((\tau E + i) + \gamma)^2}\\
%         &= \frac{(\tau E + i) + \gamma - 1}{((\tau E + i) + \gamma)^2}v + \frac{\frac{64 B_0}{\mu^2\alpha_\tau} - v}{((\tau E + i) + \gamma)^2}\\
%         &\leq \frac{v}{(\tau E + i + 1) + \gamma}
% \end{split}
% \end{equation}

% We can check it satisfies the previous assumptions regarding $\eta_\tau$:
% \begin{equation}
%     \eta_\tau \leq \eta_0 = \frac{4}{\mu\alpha_0\gamma} \leq \frac{1}{2(1+c_p)L} = \frac{1}{4L}
% \end{equation}

% \end{proof}

\subsection{Bounding $\Vert \bar{w}_{\tau E} - w^* \Vert$}
Summing from $\tau E$ to $(\tau+1)E$ we have

\begin{equation}
    \sum_{i=1}^{E}\Delta_{\tau E + i}\leq \sum_{i=0}^{E-1} (1-\frac{1}{2}\mu\eta_\tau\sum_{k=1}^N p_\tau^k \alpha_{\tau E + i}^k) \Delta_{\tau E + i} + \eta_\tau^2B_\tau + 2\eta_\tau \sum_{k=1}^N p_\tau^k s_\tau^k ( F_k(w^*) - F_k(\bar{w}_{\tau E + l}))
\end{equation}

where $B_\tau = \sum_{i=0}^{E-1} B_{\tau E + i}$, and $\bar{w}_{\tau E + l} = \text{argmin}_{\bar{w}_{\tau E + i}} \sum_{k=1}^N p_\tau^k \alpha_{\tau E + i}^k F_k(\bar{w}_{\tau E + i})$.

Reorganize it we can get
\begin{equation} \label{eq:recursive_tauE}
\begin{split}
        \Delta_{(\tau + 1) E} &\leq \Delta_{\tau E} - \frac{1}{2}\mu \eta_\tau \sum_{i=0}^{E-1}\sum_{k=1}^N p_\tau^k \alpha_{\tau E + i}^k \Delta_{\tau E + i} + \eta_\tau^2B_\tau + 2\eta_\tau \sum_{k=1}^N p_\tau^k s_\tau^k ( F_k(w^*) - F_k(\bar{w}_{\tau E + l}))
\end{split}
\end{equation}

We then seek to find a lower bound for $\Delta_{\tau E + i}$.
\begin{equation}
\begin{split}
        \sqrt{\Delta_{\tau E + i +1}} &= \Vert \bar{w}_{\tau E + i + 1} - w^* \Vert = \Vert \bar{w}_{\tau E + i + 1} - \bar{w}_{\tau E + i} + \bar{w}_{\tau E + i} - w^* \Vert \\
        &\leq \Vert \bar{w}_{\tau E + i + 1} - \bar{w}_{\tau E + i} \Vert + \sqrt{\Delta_{\tau E + i}}\\
        &= \Vert \eta_\tau \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k g_{\tau E + i}^k \Vert + \sqrt{\Delta_{\tau E + i}}
\end{split}
\end{equation}
Define $h_{\tau E + i} = \Vert \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k g_{\tau E + i}^k \Vert$.

Thus,
\begin{equation}
\begin{split}
        \sqrt{\Delta_{(\tau+1) E}} &\leq \sqrt{\Delta_{(\tau + 1)E - 1}} + \eta_\tau h_{(\tau + 1)E - 1} \\
        &\leq \dots \leq \sqrt{\Delta_{\tau E + i}} + \sum_{j=i}^{E-1}\eta_\tau h_{\tau E + j}
\end{split}
\end{equation}

\begin{equation}
\begin{split}
        \Delta_{(\tau + 1)E} &\leq \Delta_{\tau E + i} + 2\sqrt{\Delta_{\tau E + i}}(\sum_{j=i}^{E-1}\eta_\tau h_{\tau E + j}) + (\sum_{j=i}^{E-1}\eta_\tau h_{\tau E + j})^2\\
        &\leq 2\Delta_{\tau E + i} + 2(\sum_{j=i}^{E-1}\eta_\tau h_{\tau E + j})^2
\end{split}
\end{equation}

\begin{equation} \label{eq:Delta_lower_bound}
    \Delta_{\tau E + i} \geq \frac{1}{2}\Delta_{(\tau + 1)E} - (\sum_{j=i}^{E-1}\eta_\tau h_{\tau E + j})^2 \geq \frac{1}{2}\Delta_{(\tau + 1)E} - (\sum_{j=0}^{E-1}\eta_\tau h_{\tau E + j})^2
\end{equation}

Plug (\ref{eq:Delta_lower_bound}) to (\ref{eq:recursive_tauE}) we can get
\begin{equation}
\begin{split}
        (1+\frac{1}{4}\mu \eta_\tau \sum_{k=1}^N p_\tau^k s_\tau^k)\Delta_{(\tau + 1) E} \leq \Delta_{\tau E} &+ \frac{1}{2}\mu \eta_\tau^3 \sum_{k=1}^N p_\tau^k s_\tau^k (\sum_{i=0}^{E-1} h_{\tau E + i})^2 + \eta_\tau^2B_\tau \\
        &+ 2\eta_\tau \sum_{k=1}^N p_\tau^k s_\tau^k ( F_k(w^*) - F_k(\bar{w}_{\tau E + l}))
\end{split}
\end{equation}

Apply Lemma \ref{lm:grad_var}, Lemma \ref{lm:local_global_div} and Assumption \ref{asm:G2}, we have

\begin{equation}
\begin{split}
        &\mathbb{E}_\xi[h_{\tau E + i}^2] = \mathbb{E}_\xi\Vert \sum_{k=1}^N p_\tau^k\alpha_{\tau E + i}^k g_{\tau E + i}^k \Vert^2 \\
        \leq& \sum_{k=1}^N \frac{(p_\tau^k)^2}{p^k}\mathbb{E}_\xi \Vert\alpha_{\tau E + i}^kg_{\tau E + i}^k\Vert^2 \leq \sum_{k=1}^N \frac{(p_\tau^k)^2}{p^k}G^2 \alpha_{\tau E + i}^k
\end{split}
\end{equation}

\begin{equation}
\begin{split}
    &\mathbb{E}_\xi [(\sum_{i=0}^{E-1} h_{\tau E + i})^2] \leq \mathbb{E}_\xi [E \sum_{i=0}^{E-1} h_{\tau E + i}^2] \leq EG^2\sum_{k=1}^N\frac{(p_\tau^k)^2}{p^k}s_\tau^k
\end{split}
\end{equation}

\begin{equation}
\begin{split}
        \mathbb{E}_\xi &[B_\tau] = \sum_{i=0}^{E-1}\mathbb{E}_\xi[B_{\tau E + i}] = \sum_{k=1}^N (p_\tau^k)^2s_\tau^k \sigma_k^2  + 2(2+c_p)L \sum_{k=1}^N p_\tau^ks_\tau^k \Gamma_k \\
        &+(2 + \frac{\mu}{2(1+c_p)L})E(E-1)G^2 \Big(\sum_{k=1}^Np_\tau^k s_\tau^k + c_p(\sum_{k=1}^N p_\tau^k - 2)_+\sum_{k=1}^N p_\tau^ks_\tau^k \Big)
\end{split}
\end{equation}

Write $\bar{\Delta}_{\tau E + i} = \mathbb{E}_\xi[\Delta_{\tau E + i}]$,$ \bar{B}_\tau = \mathbb{E}_\xi[B_\tau]$, $\bar{H}_\tau = \mathbb{E}_\xi [(\sum_{i=0}^{E-1} h_{\tau E + i})^2]$, then

\begin{equation} \label{eq:recursive_tauE_2}
\begin{split}
        (1+\frac{1}{4}\mu \eta_\tau \sum_{k=1}^N p_\tau^k s_\tau^k)\bar{\Delta}_{(\tau + 1) E} \leq \bar{\Delta}_{\tau E} &+ \frac{1}{2}\mu \eta_\tau^3 \sum_{k=1}^Np_\tau^k s_\tau^k\bar{H}_\tau + \eta_\tau^2\bar{B}_\tau \\
        &+ 2\eta_\tau \mathbb{E}_\xi \sum_{k=1}^N p_\tau^k s_\tau^k ( F_k(w^*) - F_k(\bar{w}_{\tau E + l}))
\end{split}
\end{equation}

Let $z_\tau = 0$ indicate the event that for all $k$, $\mathbb{E}[p_\tau^ks_\tau^k] = c_\tau p^k$ for come constant $c_\tau$ that does not depend on $k$, otherwise $z_\tau^k = 1$. 

Note that if $z_\tau = 0$, then $\sum_{k=1}^N p_\tau^k s_\tau^k ( F_k(w^*) - F_k(\bar{w}_{\tau E + l})) = c_\tau(F(w^*)-F(\bar{w}_{\tau E + l})) \leq 0$. Otherwise, we have

\begin{equation}
\begin{split}
    \sum_{k=1}^N p_\tau^k s_\tau^k (F_k(w^*) - F_k(\bar{w}_{\tau E + l})) =& \sum_{k=1}^N p_\tau^k s_\tau^k ( \underbrace{F_k(w^*) - F_k^*}_{\Gamma_k} + \underbrace{F_k^* - F_k(\bar{w}_{\tau E + l}}_{\leq 0}))\\
    \leq& \sum_{k=1}^N p_\tau^k s_\tau^k \Gamma_k
\end{split}
\end{equation}

Put it together
\begin{equation}
    \sum_{k=1}^N p_\tau^k s_\tau^k ( F_k(w^*) - F_k(\bar{w}_{\tau E + l})) \leq z_\tau \sum_{k=1}^N p_\tau^k s_\tau^k \Gamma_k
\end{equation}

Assume $\eta_\tau \leq \frac{4}{\mu Ec_p} \leq \frac{4}{\mu \sum_{k=1}^N p_\tau^k s_\tau^k}$, divide both sides with $1+\frac{1}{4}\mu\eta_\tau\sum_{k=1}^N p_\tau^k s_\tau^k$ in (\ref{eq:recursive_tauE_2}) we can get

\begin{equation}
\begin{split}
        \bar{\Delta}_{(\tau + 1)E} &\leq \Big(1- \frac{\frac{1}{4}\mu\eta_\tau\sum_{k=1}^N p_\tau^k s_\tau^k}{1+\frac{1}{4}\mu\eta_\tau\sum_{k=1}^N p_\tau^k s_\tau^k} \Big)\bar{\Delta}_{\tau E} + 2 \eta_\tau^2 \bar{H}_\tau + \eta_\tau^2\bar{B}_\tau \\
        &+ 2 \eta_\tau z_\tau \sum_{k=1}^N p_\tau^k s_\tau^k \Gamma_k\\
        &\leq \Big( 1 - \frac{1}{8}\mu\eta_\tau\sum_{k=1}^N p_\tau^k s_\tau^k \Big) \bar{\Delta}_{\tau E} + \eta_\tau^2 (\bar{B}_\tau + 2\bar{H}_\tau) + 2 \eta_\tau z_\tau \sum_{k=1}^N p_\tau^k s_\tau^k \Gamma_k
\end{split}
\end{equation}

Note that $p_\tau^k$, $s_\tau^k$ are independent with $\bar{\Delta}_{\tau E}$. Taking expectation over $p_\tau^k$ and $s_\tau^k$ we get

\begin{equation}
\begin{split}
        \mathbb{E}[\bar{\Delta}_{(\tau + 1)E}] \leq \Big( 1 - \frac{1}{8}\mu\eta_\tau\mathbb{E}[\sum_{k=1}^N p_\tau^k s_\tau^k] \Big) \bar{\Delta}_{\tau E} + \eta_\tau^2 \mathbb{E}[\bar{B}_\tau + 2\bar{H}_\tau] + 2 \eta_\tau z_\tau \sum_{k=1}^N \mathbb{E}[p_\tau^k s_\tau^k] \Gamma_k
\end{split}
\end{equation}

% Assume following expectations (or conditional expectation if otherwise noted) exist or are bounded: $\mathbb{E}[p_\tau^k]$, $\mathbb{E}[p_\tau^ks_\tau^k] \neq 0$, $\mathbb{E}[(p_\tau^k)^2s_\tau^k]$, $\mathbb{E}[(\sum_{k=1}^Np_\tau^k-2)_+(\sum_{k=1}^Np_\tau^ks_\tau^k)]$. Define $D=32(E+1)\sum_{k=1}^N\mathbb{E}[p_\tau^ks_\tau^k]\Gamma_k/(\mu \mathbb{E}[\sum_{k=1}^Np_\tau^ks_\tau^k])$, $M_\tau = \sum_{t=0}^{\tau - 1} z_\tau$ (so $M_0 = 0$), we have the following theorem:

% \begin{theorem} \label{tm:convergence0}
% \begin{equation}
%     \mathbb{E}[\bar{\Delta}_{\tau E}] \leq \frac{v + M_\tau D}{\tau E + \gamma}
% \end{equation}
% \end{theorem}

% \begin{proof}
% We prove by induction. Let $\eta_\tau = \frac{8}{\mu \mathbb{E}[\sum_{k=1}^Np_\tau^ks_\tau^k]}\frac{E+1}{\tau E + \gamma}$, where $\gamma = \max \{16(E+1)(1+c_p)L/(\mu \mathbb{E}[\sum_{k=1}^Np_\tau^ks_\tau^k]), 2(E+1)Ec_p/\mathbb{E}[\sum_{k=1}^Np_\tau^ks_\tau^k] \}, v = \max \{(E+1)^2\max_\tau\mathbb{E}[\bar{B}_\tau+2\bar{H}_\tau], \gamma \mathbb{E}[\bar{\Delta}_0] \}$. Initially, $\frac{v}{\gamma} \geq \bar{\Delta}_0$. Suppose $\mathbb{E}[\bar{\Delta}_{\tau E}] \leq \frac{v+M_\tau D}{\tau E + \gamma}$, then

% \begin{equation}
% \begin{split}
%         \mathbb{E}[\bar{\Delta}_{(\tau + 1)E}] &\leq \frac{\tau E + \gamma - E}{\tau E + \gamma}\frac{v+M_\tau D}{\tau E + \gamma} + \frac{(E+1)^2\mathbb{E}[\bar{B}_\tau+2\bar{H}_\tau]-v-M_\tau D}{(\tau E + \gamma)^2}+\frac{\frac{1}{2}z_\tau D}{\tau E + \gamma} \\
%         &\leq \frac{\tau E + \gamma - E}{(\tau E + \gamma)^2-E^2}(v+M_\tau D) + \frac{\frac{1}{2}z_\tau D}{(\tau + 1) E + \gamma} \frac{(\tau + 1) E + \gamma}{\tau E + \gamma}\\
%         &\leq \frac{v+M_\tau D}{(\tau + 1)E + \gamma} + \frac{z_\tau D}{(\tau + 1)E + \gamma} = \frac{v+M_{\tau + 1}D}{(\tau + 1)E + \gamma}
% \end{split}
% \end{equation}

% Thus $\bar{\Delta}_{(\tau + 1)E } \leq \frac{v+M_{\tau + 1}D}{(\tau + 1)E + \gamma}$.

% We can check it satisfies the previous assumptions regarding $\eta_\tau$:

% \begin{equation}
% \begin{split}
%         &\eta_\tau \leq \eta_0 = \frac{8(E+1)/(\mu \mathbb{E}[\sum_{k=1}^Np_\tau^ks_\tau^k]}{\gamma}\\ \leq& \frac{8(E+1)/(\mu \mathbb{E}[\sum_{k=1}^Np_\tau^ks_\tau^k])}{16(E+1)(1+c_p)L/(\mu \mathbb{E}[\sum_{k=1}^Np_\tau^ks_\tau^k])} = \frac{1}{2(1+c_p)L}
% \end{split}
% \end{equation}

% \begin{equation}
%     \eta_\tau \leq \eta_0 = \frac{8(E+1)}{\mu\mathbb{E}[\sum_{k=1}^Np_\tau^ks_\tau^k]\gamma} \leq \frac{8(E+1)}{2\mu(E+1)Ec_p} = \frac{4}{\mu Ec_p}
% \end{equation}

% \end{proof}

Assume following expectations (or conditional expectation if otherwise noted) exist or are bounded: $\mathbb{E}[p_\tau^k]$, $\mathbb{E}[p_\tau^ks_\tau^k] \neq 0$, $\mathbb{E}[(p_\tau^k)^2s_\tau^k]$, $\mathbb{E}[(\sum_{k=1}^Np_\tau^k-2)_+(\sum_{k=1}^Np_\tau^ks_\tau^k)]$.

\begin{theorem} \label{tm:convergence0}
\begin{equation}
    \mathbb{E}[\bar{\Delta}_{\tau E}] \leq \frac{M_\tau D}{\tau E + \gamma} + \frac{V_\tau}{\left(\tau E + \gamma\right)^2}
\end{equation}

where $D=32E\sum_{k=1}^N\mathbb{E}[p_\tau^ks_\tau^k]\Gamma_k/(\mu \mathbb{E}[\sum_{k=1}^Np_\tau^ks_\tau^k])$, $M_\tau = \sum_{t=0}^{\tau - 1} z_\tau$ (so $M_0 = 0$), $\gamma = \max \{32E(1+c_p)L/(\mu \mathbb{E}[\sum_{k=1}^Np_\tau^ks_\tau^k]), 4E^2c_p/\mathbb{E}[\sum_{k=1}^Np_\tau^ks_\tau^k] \}$, $V_\tau = \max\left\{\gamma^2 \mathbb{E}[\bar{\Delta}_0], \left(\frac{16E}{\mu}\right)^2\sum_{t=0}^{\tau - 1} \frac{\mathbb{E}[\bar{B}_t + 2\bar{H}_t]}{\left(\mathbb{E}[\sum_{k=1}^Np_t^ks_t^k]\right)^2} \right\}$
\end{theorem}

\begin{proof}
We prove by induction. Let $\eta_\tau = \frac{8}{\mu \mathbb{E}[\sum_{k=1}^Np_\tau^ks_\tau^k]}\frac{2E}{(\tau+1) E + \gamma}$. Initially, $\frac{V_0}{\gamma^2} \geq \mathbb{E}[\bar{\Delta}_0]$. Suppose $\mathbb{E}[\bar{\Delta}_{\tau E}] \leq \frac{M_\tau D}{\tau E + \gamma} + \frac{V_\tau}{\left(\tau E + \gamma\right)^2}$, then

\begin{equation}
\begin{split}
        &\mathbb{E}[\bar{\Delta}_{(\tau + 1)E}] \leq \frac{\tau E + \gamma - E}{(\tau+1) E + \gamma}\left(\frac{M_\tau D}{\tau E + \gamma} + \frac{V_\tau}{\left(\tau E + \gamma\right)^2}\right) + \frac{(16E)^2\mathbb{E}[\bar{B}_\tau+2\bar{H}_\tau]}{(\mu\mathbb{E}[\sum_{k=1}^Np_\tau^ks_\tau^k])^2\left((\tau + 1) E + \gamma\right)^2}+\frac{z_\tau D}{(\tau+1) E + \gamma} \\
        \leq& \frac{(\tau E + \gamma - E)M_\tau D}{(\tau E + \gamma)^2-E^2} + \frac{\tau E + \gamma - E}{(\tau E + \gamma)^2-E^2}\frac{V_\tau}{(\tau+1) E + \gamma} + \frac{(16E)^2\mathbb{E}[\bar{B}_\tau+2\bar{H}_\tau]}{(\mu\mathbb{E}[\sum_{k=1}^Np_\tau^ks_\tau^k])^2\left((\tau + 1) E + \gamma\right)^2} + \frac{z_\tau D}{(\tau + 1) E + \gamma}\\
        \leq& \frac{M_\tau D}{(\tau + 1)E + \gamma} + \frac{V_\tau}{\left((\tau + 1)E + \gamma\right)^2} + \frac{(16E)^2\mathbb{E}[\bar{B}_\tau+2\bar{H}_\tau]}{(\mu\mathbb{E}[\sum_{k=1}^Np_\tau^ks_\tau^k])^2\left((\tau + 1) E + \gamma\right)^2} + \frac{z_\tau D}{(\tau + 1)E + \gamma} \\
        =& \frac{M_{\tau + 1} D}{(\tau + 1)E + \gamma} + \frac{V_{\tau + 1}}{\left((\tau + 1)E + \gamma\right)^2}
\end{split}
\end{equation}

Thus $\bar{\Delta}_{(\tau + 1)E } \leq \frac{M_{\tau + 1} D}{(\tau + 1)E + \gamma} + \frac{V_{\tau + 1}}{\left((\tau + 1)E + \gamma\right)^2}$.

We can check it satisfies the previous assumptions regarding $\eta_\tau$:

\begin{equation}
\begin{split}
        &\eta_\tau \leq \eta_0 = \frac{16E/(\mu \mathbb{E}[\sum_{k=1}^Np_\tau^ks_\tau^k])}{E + \gamma}\\ 
        \leq& \frac{16E/(\mu \mathbb{E}[\sum_{k=1}^Np_\tau^ks_\tau^k])}{32E(1+c_p)L/(\mu \mathbb{E}[\sum_{k=1}^Np_\tau^ks_\tau^k])} = \frac{1}{2(1+c_p)L}
\end{split}
\end{equation}

\begin{equation}
    \eta_\tau \leq \eta_0 = \frac{16E/(\mu \mathbb{E}[\sum_{k=1}^Np_\tau^ks_\tau^k])}{E + \gamma} \leq \frac{16E/(\mu \mathbb{E}[\sum_{k=1}^Np_\tau^ks_\tau^k])}{4E^2c_p/( \mathbb{E}[\sum_{k=1}^Np_\tau^ks_\tau^k])} = \frac{4}{\mu Ec_p}
\end{equation}

\end{proof}

\begin{corollary} \label{cor:M_tau}
If $M_\tau = O(\tau)$, the learning will not converge to the global optimal.
\end{corollary}



\section{Three schemes and four cases}
To avoid confusion, we say a client is inactive(active) in round $\tau$ if $s_\tau^k = 0$ ($s_\tau^k \neq 0$), and say a client is incomplete(complete) if $0 \leq s_\tau^k < E$ ($s_\tau^k = E$). We say a client fails if it is inactive.

We will discuss three different aggregation schemes. Theorem \ref{tm:convergence0} works for all of them.

\begin{itemize}[leftmargin=*]
    \item Scheme A (extension of \emph{FedAvg}): only aggregate clients who complete all $E$ local epochs, with weight $p_\tau^k = \frac{Np^k}{K_\tau}q_\tau^k$, where $K_\tau$ is the number of complete devices, $q_\tau^k \in \{0,1\}$ denotes if client $k$ is complete, i.e., it completes $E$ epochs. If $K_\tau=0$, this round is discarded.
    \item Scheme B: Allow clients to upload incomplete work, with fixed weight $p_\tau^k = p^k$.
    \item Scheme C: Allow clients to upload incomplete work, with adaptive weight $p_\tau^k =  \frac{E}{s_\tau^k}p^k$, or 0 if $s_\tau^k = 0$.
\end{itemize}

In the meanwhile, there are four scenarios regarding the distribution of $s_\tau^k$.
\begin{itemize}[leftmargin=*]
    \item Case I: No failure, homogeneous $s_\tau^k$.
    \item Case II: No failure, heterogeneous $s_\tau^k$.
    \item Case III: With failure, homogeneous $s_\tau^k$.
    \item Case IV: With failure, heterogeneous $s_\tau^k$.
\end{itemize}

Let $y_\tau = 1$ denote if there exists any inactive client in round $\tau$, and let $y_\tau^k$ indicate if client $k$ is inactive in round $\tau$. So $\mathbb{P}(y_\tau^k = 0|y_\tau = 0) = 1$.

There will then be total 12 combinations:
\begin{center}
\begin{tabular}{ |c|c|c| } 
 \hline
          & Case I & Case II \\
 \hline
 Scheme A & $O\left(\frac{E^3N^2\sum_{t=0}^{\tau - 1}\mathbb{E}[\frac{1}{K_\tau}|K_\tau \neq 0]}{(\tau E + EN)^2}\right)$ & N/A  \\ 
 \hline
 Scheme B & $O\left(\frac{\left(E^4 + E^2\sum_{k=1}^N(p^k\sigma_k)^2\right)\sum_{t=0}^{\tau-1}\frac{1}{\mathbb{E}[s_t]}}{\left(\tau E + E\right)^2}\right)$ & N/A  \\ 
 \hline
 Scheme C & $O\left(\frac{\left(E^5 + E^2\sum_{k=1}^N(p^k\sigma_k)^2\right)\sum_{t=0}^{\tau - 1}\mathbb{E}\left[\frac{1}{s_t}\right]}{\left(\tau E + E^2\right)^2}\right)$ & $O\left(\frac{E^5\sum_{t=0}^{\tau-1}\sum_{k=1}^Np^k\mathbb{E}\Big[\frac{1}{s_t^k}\Big] + E^2\sum_{t=0}^{\tau-1}\sum_{k=1}^N (p^k\sigma_k)^2\mathbb{E}\Big[\frac{1}{s_t^k}\Big]}{(\tau E + E^2)^2}\right)$  \\ 
 \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{ |c|c|c| } 
 \hline
          & Case III & Case IV \\
 \hline
 Scheme A & Same as Case I & N/A  \\ 
 \hline
 Scheme B & Same as Case I & N/A  \\ 
 \hline
 Scheme C & Same as Case I & $O\left(\frac{\sum_{t=0}^{\tau - 1}y_\tau D}{\tau E + E^2} + \frac{E^5\sum_{t=0}^{\tau-1}\sum_{k=1}^Np^k\mathbb{P}(y_t^k=0)\mathbb{E}\Big[\frac{1}{s_t^k}\Big] + E^2\sum_{t=0}^{\tau-1}\sum_{k=1}^N (p^k\sigma_k)^2\mathbb{P}(y_t^k=0)\mathbb{E}\Big[\frac{1}{s_t^k}\Big]}{(\tau E + E^2)^2}\right)$ \\ 
 \hline
\end{tabular}
\end{center}

\section{Scheme A}
In Scheme A, we only consider clients whose $s_\tau^k = E$. Let $K_\tau$ be the number of complete clients in round $\tau$. Let $q_\tau^k$ be an indicator denoting if client $k$ is complete in round $\tau$. Thus, $K_\tau = \sum_{k=1}^N q_\tau^k$.

\subsection{Case I}
Obviously $q_\tau^k$'s are homogeneous when $s_\tau^k$'s are homogeneous. We have $\mathbb{E}[q_\tau^k] = q_\tau$, where $q_\tau = \mathbb{P}(s_\tau = E)$. We then have $\mathbb{P}(K_\tau = 0) = (1-q_\tau)^N$.

When choosing $p_\tau^k = \frac{Np^k}{K_\tau}q_\tau^k$, $c_p = N$. Note that by the definition of $q_\tau^k$, we have $q_\tau^k s_\tau^k = Eq_\tau^k$, so $\mathbb{E}[p_\tau^ks_\tau^k] = E\mathbb{E}[p_\tau^k]$. Similarly, we can replace all $s_\tau^k$ terms with $E$. When then only focus on $\mathbb{E}[p_\tau^k]$:
\begin{equation}
\begin{split}
        &\mathbb{E}_q[p_\tau^k|K_\tau \neq 0] = Np^k\mathbb{E}_q\Big[\frac{q_\tau^k}{\sum_{i=1}^N q_\tau^i}\Big | K_\tau \neq 0]\\
        =&Np^k\sum_{i=0}^{N-1}\frac{1}{1+i} {N-1 \choose i} \frac{(q_\tau)^i(1-q_\tau)^{N-1-i}q_\tau}{1-(1-q_\tau)^N}\\
        =&Np^k\sum_{i=1}^{N}\frac{1}{i}{N-1 \choose i-1}\frac{(q_\tau)^i(1-q_\tau)^{N-i}}{1-(1-q_\tau)^N} = Np^k\sum_{i=1}^{N}\frac{1}{i}\frac{(N-1)!}{(i-1)!(N-i)!}\frac{(q_\tau)^i(1-q_\tau)^{N-i}}{1-(1-q_\tau)^N}\\
        =&p^k\sum_{i=1}^N {N \choose i}\frac{(q_\tau)^i(1-q_\tau)^{N-i}}{1-(1-q_\tau)^N} = p^k \frac{1-{N \choose 0}(q_\tau)^0(1-q_\tau)^N}{1-(1-q_\tau)^N} = p^k
\end{split}
\end{equation}

Similarly,
\begin{equation}
\begin{split}
        &\mathbb{E}_q[(p_\tau^k)^2|K_\tau \neq 0] = (Np^k)^2\mathbb{E}_q\Big[\frac{q_\tau^k}{(\sum_{i=1}^N q_\tau^i)^2}\Big | K_\tau \neq 0]\\
        =&(Np^k)^2\sum_{i=0}^{N-1}\frac{1}{(1+i)^2} {N-1 \choose i} \frac{(q_\tau)^i(1-q_\tau)^{N-1-i}q_\tau}{1-(1-q_\tau)^N}\\
        =&(Np^k)^2\sum_{i=1}^{N}\frac{1}{i^2}{N-1 \choose i-1}\frac{(q_\tau)^i(1-q_\tau)^{N-i}}{1-(1-q_\tau)^N} = N(p^k)^2\sum_{i=1}^{N}\frac{1}{i}{N \choose i}\frac{(q_\tau)^i(1-q_\tau)^{N-i}}{1-(1-q_\tau)^N}\\
        =&N(p^k)^2\mathbb{E}\Big[\frac{1}{K_\tau}|K_\tau \neq 0\Big]
\end{split}
\end{equation}

It is possible that $\sum_{k=1}^N p_\tau^k > 2$, so we need to calculate $\mathbb{E}[p_\tau^kp_\tau^l|K_\tau \neq 0]$
\begin{equation}
\begin{split}
    &\mathbb{E}_q[p_\tau^kp_\tau^l|K_\tau \neq 0] = N^2p^kp^l\mathbb{E}\Big[\frac{q_\tau^kq_\tau^l}{(\sum_{i=1}^Nq_\tau^i)^2}|K_\tau \neq 0\Big]\\
    =&N^2p^kp^l \sum_{i=0}^{N-2}\frac{1}{(2+i)^2}{N-2 \choose i}\frac{(q_\tau)^i(1-q_\tau)^{N-2-i}(q_\tau)^2}{1-(1-q_\tau)^N}\\
    =& \frac{N}{N-1}p^kp^l\sum_{i=2}^N\frac{i-1}{i}{N \choose i}\frac{(q_\tau)^i(1-q_\tau)^{N-i}}{1-(1-q_\tau)^N} = \frac{N}{N-1}p^kp^l\mathbb{E}\Big[1-\frac{1}{K_\tau}|K_\tau \neq 0\Big]
\end{split}
\end{equation}

For all $k$ and $\tau$, $\mathbb{E}[p_\tau^ks_\tau^k|K_\tau \neq 0] = Ep^k$, thus $z_\tau = 0, M_\tau = 0$ for all $k,\tau$.

Therefore,
$\mathbb{E}[\bar{B}_\tau] = \Theta(E^3N^2\mathbb{E}[\frac{1}{K_\tau}|K_\tau \neq 0]+E\sum_{k=1}^N(p^k\sigma_k)^2), \mathbb{E}[\bar{H}_\tau] = \Theta(E^2N\mathbb{E}[\frac{1}{K_\tau}|K_\tau \neq 0])$, and we have
$\gamma = \Theta(EN)$, hence $V_\tau = \Theta(E^3N^2\sum_{t=0}^{\tau - 1}\mathbb{E}[\frac{1}{K_\tau}|K_\tau \neq 0])$. Plug them into Theorem \ref{tm:convergence0}, we can get an asymptotic rate of $O\left(\frac{E^3N^2\sum_{t=0}^{\tau - 1}\mathbb{E}[\frac{1}{K_\tau}|K_\tau \neq 0]}{(\tau E + EN)^2}\right)$. The actual rate has to scale by the probability that $K_\tau \neq 0$, which is trivial when $N$ goes large.

\subsection{Case II}
When $s_\tau^k$'s (i.e., $q_\tau^k$'s) are heterogeneous, generally $\mathbb{E}[p_\tau^k] \neq p^k$, furthermore, we may have $z_\tau = 1$ for all $\tau$.

To see this, consider an example where a client $k_0$ has $q_\tau^{k_0} = 1$, i.e. $\mathbb{P}(s_\tau^k = E) = 1$, whereas all the rest clients have $\mathbb{E}[q_\tau^k] = q_\tau$, then we can show that

\begin{equation}
    \mathbb{E}_q[p_\tau^{k_0}|K_\tau \neq 0] = \mathbb{E}_q[p_\tau^{k_0}] = Np^{k_0}\mathbb{E}_q\Big[\frac{q_\tau^{k_0}}{(\sum_{i=1}^N q_\tau^i)^2}\Big] = p^{k_0}\frac{1-(1-q_\tau)^N}{q_\tau}
\end{equation}

and for $k \neq k_0$

\begin{equation}
\begin{split}
    &\mathbb{E}_q[p_\tau^{k}|K_\tau \neq 0] = \mathbb{E}_q[p_\tau^{k}] = Np^{k}\mathbb{E}_q\Big[\frac{q_\tau^{k}}{(\sum_{i=1}^N q_\tau^i)^2}\Big] \\
    =&\frac{p^k}{(N-1)q_\tau}\sum_{i=2}^N(i-1){N \choose i}(q_\tau)^i(1-q_\tau)^{N-i}\\
    =&\frac{p^k}{(N-1)q_\tau}\Big(Nq_\tau - Nq_\tau(1-q_\tau)^{N-1} - (1-(1-q_\tau)^N - Nq_\tau(1-q_\tau)^{N-1})\Big)\\
    =&p^k\frac{Nq_\tau+(1-q_\tau)^N-1}{(N-1)q_\tau}
\end{split}
\end{equation}

Thus, different $k$ will have different ratio of $\mathbb{E}[p_\tau^ks_\tau^k/p^k]=E\mathbb{E}[p_\tau^k/p^k]$, which indicates $z_\tau = 1$.

Since this is true for all $\tau$, we have $M_\tau = \tau$, thus according to Corollary \ref{cor:M_tau}, the learning will not converge to the global optimal.

\subsection{Case III and IV}
Note that inactiveness is a special case of incompleteness, Scheme A has the same convergence results as in Case I and II.

\section{Scheme B}
In Scheme B, $p_\tau^k = p^k$ is a fixed number, so we only need to take expectation over $s_\tau^k$, and $c_p = 1$. Since $\sum_{k=1}^N p^k = 1 < 2$, we can bound $\mathbb{E}[(\sum_{k=1}^Np_\tau^k-2)_+(\sum_{k=1}^Np_\tau^ks_\tau^k)] < 0$.
\subsection{Case I}
When $s_\tau^k$'s are homogeneous, i.e. $s_\tau^k \overset{iid}{\sim} s_\tau$, then $\mathbb{E}[p_\tau^ks_\tau^k]/p^k = \mathbb{E}[s_\tau]$. This is the same for all $k$, thus $z_\tau = 0$ and $M_\tau = 0$.

Moreover, we have $\mathbb{E}[\bar{B}_\tau] = \Theta(E^2\mathbb{E}[s_\tau] + \mathbb{E}[s_\tau]\sum_{k=1}^N(p^k\sigma_k)^2)$, $\mathbb{E}[\bar{H}_\tau] = \Theta(E\mathbb{E}[s_\tau])$, $\gamma = \Theta(E^2/\mathbb{E}[s_\tau])$, $V_\tau = \Theta\left(\left(E^4 + E^2\sum_{k=1}^N(p^k\sigma_k)^2\right)\sum_{t=0}^{\tau-1}\mathbb{E}[s_t]\right)$, which gives an asymptotic convergence rate of $O\left(\frac{\left(E^4 + E^2\sum_{k=1}^N(p^k\sigma_k)^2\right)\sum_{t=0}^{\tau-1}\frac{1}{\mathbb{E}[s_t]}}{\left(\tau E + E\right)^2}\right)$.

\subsection{Case II}
When $s_\tau^k$'s are heterogeneous, $\mathbb{E}[p_\tau^ks_\tau^k]/p^k = \mathbb{E}[s_\tau^k]$ varies with $k$. Thus, $z_\tau = 1$ and $M_\tau = \tau$. Therefore, the algorithm will not converge as per Corollary \ref{cor:M_tau}.

\subsection{Case III}
\begin{equation*}
    \mathbb{E}[p_\tau^ks_\tau^k] = p^k\mathbb{E}[\mathbb{E}[s_\tau^k|y_\tau^k]] = p^k\mathbb{P}(y_\tau^k = 0)\mathbb{E}[s_\tau^k|y_\tau^k = 0]
\end{equation*}
In the homogeneous case, the ratio $\mathbb{E}[p_\tau^ks_\tau^k]/p^k$ is the same for all $k$. So $z_\tau = 0$ and $M_\tau = 0$.

The convergence rate is the same as Case II, except for replacing $\mathbb{E}[s_\tau]$ with $\mathbb{P}(y_\tau = 0)\mathbb{E}[s_\tau|y_\tau^k = 0]$


\subsection{Case IV}
Since $\mathbb{E}[p_\tau^ks_\tau^k] = p^k\mathbb{P}(y_\tau^k = 0)\mathbb{E}[s_\tau^k|y_\tau^k = 0]$. In the heterogeneous case, $\mathbb{P}(y_\tau^k = 0)\mathbb{E}[s_\tau^k|s_\tau^k\neq 0]$ generally varies with $k$, unless the heterogeneity of $y_\tau^k$ can perfectly offset the heterogeneity of $s_\tau^k$. So $z_\tau = 1$ and $M_\tau = \tau$. The learning will not converge to the global optimal.

\section{Scheme C}
In Scheme C, $p_\tau^k = \frac{Ep^k}{s_\tau^k}$, so $c_p = E$. It is possible that $\sum_{k=1}^Bp_\tau^k > 2$, so we need to calculate $\mathbb{E}\Big[(\sum_{k=1}^Np_\tau^k)(\sum_{k=1}^Np_\tau^ks_\tau^k)\Big]$.

\subsection{Case I}
When $s_\tau^k$'s are homogeneous, $\mathbb{E}[p_\tau^ks_\tau^k]/p^k = E$ for all $k$. Thus, $z_\tau = 0, M_\tau = 0$.

Moreover, we have
\begin{equation}
    \mathbb{E}[\sum_{k=1}^N p_\tau^k] = E\mathbb{E}\Big[\frac{1}{s_\tau}\Big]
\end{equation}
\begin{equation}
    \mathbb{E}[\sum_{k=1}^N (p_\tau^k)^2] = \Big(E\mathbb{E}\Big[\frac{1}{s_\tau}\Big]\Big)^2\sum_{k=1}^N (p^k)^2
\end{equation}
\begin{equation}
    \mathbb{E}[\sum_{k=1}^N (p_\tau^k)^2s_\tau^k] = E^2\mathbb{E}\Big[\frac{1}{s_\tau}\Big] \sum_{k=1}^N (p^k)^2
\end{equation}

\begin{equation}
    \mathbb{E}\Big[(\sum_{k=1}^Np_\tau^k)(\sum_{k=1}^Np_\tau^ks_\tau^k)\Big] = E^2\mathbb{E}\Big[\frac{1}{s_\tau}\Big]
\end{equation}

Therefore, we have $\mathbb{E}[\bar{B}_\tau] = \Theta\Big(E^5\mathbb{E}\left[\frac{1}{s_\tau}\right] + E^2\mathbb{E}\left[\frac{1}{s_\tau}\right]\sum_{k=1}^N(p^k\sigma_k)^2 \Big)$, $\mathbb{E}[\bar{H}_\tau] = \Theta\Big(E^3\mathbb{E}\Big[\frac{1}{s_\tau}\Big]\Big)$, $\gamma = \Theta(E^2)$, $V_\tau = \Theta\left(\left(E^5 + E^2\sum_{k=1}^N(p^k\sigma_k)^2\right)\sum_{t=0}^{\tau - 1}\mathbb{E}\left[\frac{1}{s_t}\right]\right)$, which yields a convergence rate of $O\left(\frac{\left(E^5 + E^2\sum_{k=1}^N(p^k\sigma_k)^2\right)\sum_{t=0}^{\tau - 1}\mathbb{E}\left[\frac{1}{s_t}\right]}{\left(\tau E + E^2\right)^2}\right)$.

\subsection{Case II}
When $s_\tau^k$'s are homogeneous, we still have $\mathbb{E}[p_\tau^ks_\tau^k]/p^k = E$ for all $k$. Thus, $z_\tau = 0, M_\tau = 0$.

Moreover,
\begin{equation}
    \mathbb{E}[\sum_{k=1}^N p_\tau^k] = E\sum_{k=1}^Np^k\mathbb{E}\Big[\frac{1}{s_\tau^k}\Big]
\end{equation}
\begin{equation}
    \mathbb{E}[\sum_{k=1}^N (p_\tau^k)^2] = E^2\sum_{k=1}^N \Big(p^k\mathbb{E}\Big[\frac{1}{s_\tau^k}\Big]\Big)^2
\end{equation}
\begin{equation}
    \mathbb{E}[\sum_{k=1}^N (p_\tau^k)^2s_\tau^k] = E^2\sum_{k=1}^N (p^k)^2\mathbb{E}\Big[\frac{1}{s_\tau^k}\Big] 
\end{equation}

\begin{equation}
    \mathbb{E}\Big[(\sum_{k=1}^Np_\tau^k)(\sum_{k=1}^Np_\tau^ks_\tau^k)\Big] = E^2\sum_{k=1}^Np^k\mathbb{E}\Big[\frac{1}{s_\tau^k}\Big]
\end{equation}

$\mathbb{E}[\bar{B}_\tau] = \Theta\Big(E^5\sum_{k=1}^Np^k\mathbb{E}\Big[\frac{1}{s_\tau^k}\Big] + E^2\sum_{k=1}^N (p^k\sigma_k)^2\mathbb{E}\Big[\frac{1}{s_\tau^k}\Big] \Big), \mathbb{E}[\bar{H}_\tau] = \Theta\Big( E^3\sum_{k=1}^Np^k\mathbb{E}\Big[\frac{1}{s_\tau^k}\Big]\Big)$, $\gamma = \Theta(E^2)$, $V_\tau = \Theta\Big(E^5\sum_{t=0}^{\tau-1}\sum_{k=1}^Np^k\mathbb{E}\Big[\frac{1}{s_t^k}\Big] + E^2\sum_{t=0}^{\tau-1}\sum_{k=1}^N (p^k\sigma_k)^2\mathbb{E}\Big[\frac{1}{s_t^k}\Big]\Big)$. Thus, the convergence rate is $O\left(\frac{E^5\sum_{t=0}^{\tau-1}\sum_{k=1}^Np^k\mathbb{E}\Big[\frac{1}{s_t^k}\Big] + E^2\sum_{t=0}^{\tau-1}\sum_{k=1}^N (p^k\sigma_k)^2\mathbb{E}\Big[\frac{1}{s_t^k}\Big]}{(\tau E + E^2)^2}\right)$

\subsection{Case III}
When $y_\tau = 1$,
\begin{equation}
    \mathbb{E}[p_\tau^ks_\tau^k] = \mathbb{P}(y_\tau^k = 0)Ep^k
\end{equation}
So $z_\tau = 0$.

When $y_\tau = 0$, we also have $z_\tau = 0$. So $M_\tau = 0$.

The convergence rate is the same as Case I, except for multiplying $V_\tau$ with $\mathbb{P}(y_\tau = 0)$

\subsection{Case IV}
We still have $z_\tau = 0$ when $y_\tau = 0$. But for $y_\tau = 1$, it doesn't have to hold. So $M_\tau = \sum_{t=0}^{\tau - 1}y_\tau$.


% \subsection{Adapting $p_\tau^k$}
% Let
% \begin{equation}
%     p_\tau^k =
%     \begin{cases}
%     \frac{E}{s_\tau^k}p^k &s_\tau^k \neq 0\\
%     0 &\textrm{otherwise}
%     \end{cases}\;\;\;\;\;
%     z_\tau^k =
%     \begin{cases}
%     1 &s_\tau^k = 0\\
%     0 &s_\tau^k > 0
%     \end{cases}\;\;\;\;\;
%     z_\tau =
%     \begin{cases}
%     1 &\sum_{k=1}^N z_\tau^k > 0\\
%     0 &\textrm{otherwise}
%     \end{cases}
% \end{equation}

% Thus, $p_\tau^k s_\tau^k = Ep^k (1-z_\tau^k), c_p = E$.

% Note that if $z_\tau = 0$, i.e., every client completes at least one local epoch during round $\tau$, then $\sum_{k=1}^N p_\tau^k s_\tau^k ( F_k(w^*) - F_k(\bar{w}_{\tau E + l})) = E(F(w^*)-F(\bar{w}_{\tau E + l})) \leq 0$. Otherwise, we have

% \begin{equation}
% \begin{split}
%     \sum_{k=1}^N p_\tau^k s_\tau^k (F_k(w^*) - F_k(\bar{w}_{\tau E + l})) =& \sum_{k=1}^N p_\tau^k s_\tau^k ( \underbrace{F_k(w^*) - F_k^*}_{\Gamma_k} + \underbrace{F_k^* - F_k(\bar{w}_{\tau E + l}}_{\leq 0}))\\
%     \leq& \sum_{k=1}^N Ep^k(1-z_\tau^k)\Gamma_k
% \end{split}
% \end{equation}

% Put it together
% \begin{equation}
%     \sum_{k=1}^N p_\tau^k s_\tau^k ( F_k(w^*) - F_k(\bar{w}_{\tau E + l})) \leq z_\tau E \sum_{k=1}^N p^k(1-z_\tau^k)\Gamma_k
% \end{equation}

% \subsection{Homogeneous Failures}
% Assume $\mathbb{E}[z_\tau^k]$ does not change over time. Along with the condition $p_\tau^k/p^k \leq c_p = E$, we can bound $\bar{B}_\tau \leq B$, $\bar{H}_\tau \leq H$.

% Write $\bar{q}_z = \mathbb{E}_{z}\sum_{k=1}^N p^k(1-z_\tau^k)$. Further assume $\frac{1}{4}\mu E \eta_\tau\bar{q}_z \leq 1$. Reorganize (\ref{eq:recursive_tauE_2}) we can get

% \begin{equation}
% \begin{split}
%         \bar{\Delta}_{(\tau + 1)E} &\leq \Big(1- \frac{\frac{1}{4}\mu  E\bar{q}_z\eta_\tau}{1+\frac{1}{4}\mu E\bar{q}_z\eta_\tau} \Big)\bar{\Delta}_{\tau E} + \frac{1}{2}\mu E \eta_\tau^3 \bar{q}_z\bar{H} + \eta_\tau^2\bar{B} \\
%         &+ 2 Ez_\tau \eta_\tau \sum_{k=1}^N p^k(1-z_\tau^k)\Gamma_k\\
%         &\leq \Big( 1 - \frac{1}{8}\mu  E\bar{q}_z\eta_\tau \Big) \bar{\Delta}_{\tau E} + \eta_\tau^2 (\bar{B} + 2\bar{H}) + 2Ez_\tau\eta_\tau\Gamma
% \end{split}
% \end{equation}

% Let define $D=32\Gamma(E+1)/(\mu \bar{q}_z)$, $M_\tau = \sum_{t=0}^{\tau - 1} z_\tau$ (so $M_0 = 0$), we have the following theorem:

% \begin{theorem}
% \begin{equation}
%     \bar{\Delta}_{\tau E} \leq \frac{v + M_\tau D}{\tau E + \gamma}
% \end{equation}
% \end{theorem}

% \begin{proof}
% We prove by induction. Let $\eta_\tau = \frac{8}{\mu E \bar{q}_z}\frac{E+1}{\tau E + \gamma}$, where $\gamma = \max \{16(E+1)^2L/(\mu E\bar{q}_z), 2(E+1) \}, v = \max \{(E+1)^2(\bar{B}+2\bar{H}), \gamma \bar{\Delta}_0 \}$. Initially, $\frac{v}{\gamma} \geq \bar{\Delta}_0$. Suppose $\bar{\Delta}_{\tau E} \leq \frac{v+M_\tau D}{\tau E + \gamma}$, then

% \begin{equation}
% \begin{split}
%         \bar{\Delta}_{(\tau + 1)E} &\leq \frac{\tau E + \gamma - E}{\tau E + \gamma}\frac{v+M_\tau D}{\tau E + \gamma} + \frac{(E+1)^2(\bar{B}+2\bar{H})-v-M_\tau D}{(\tau E + \gamma)^2}+\frac{\frac{1}{2}z_\tau D}{\tau E + \gamma} \\
%         &\leq \frac{\tau E + \gamma - E}{(\tau E + \gamma)^2-E^2}(v+M_\tau D) + \frac{\frac{1}{2}z_\tau D}{(\tau + 1) E + \gamma} \frac{(\tau + 1) E + \gamma}{\tau E + \gamma}\\
%         &\leq \frac{v+M_\tau D}{(\tau + 1)E + \gamma} + \frac{z_\tau D}{(\tau + 1)E + \gamma} = \frac{v+M_{\tau + 1}D}{(\tau + 1)E + \gamma}
% \end{split}
% \end{equation}

% Thus $\bar{\Delta}_{(\tau + 1)E } \leq \frac{v+M_{\tau + 1}D}{(\tau + 1)E + \gamma}$.

% We can check it satisfies the previous assumptions regarding $\eta_\tau$:

% \begin{equation}
%     \eta_\tau \leq \eta_0 = \frac{8(E+1)/(\mu E \bar{q}_z)}{\gamma} \leq \frac{8(E+1)/(\mu E \bar{q}_z)}{16(E+1)^2L/(\mu E\bar{q}_z)} = \frac{1}{2(1+c_p)L}
% \end{equation}

% \begin{equation}
%     \frac{1}{4}\mu E\eta_\tau \bar{q}_z = \frac{2(E+1)}{\tau E + \gamma} \leq \frac{2(E+1)}{\gamma} \leq 1
% \end{equation}

% \end{proof}

==> reference.tex <==
\section*{References}

References follow the acknowledgments. Use unnumbered first-level heading for
the references. Any choice of citation style is acceptable as long as you are
consistent. It is permissible to reduce the font size to \verb+small+ (9 point)
when listing the references.
{\bf Note that the Reference section does not count towards the eight pages of content that are allowed.}
\medskip

\small

[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms for
connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and T.K.\ Leen
(eds.), {\it Advances in Neural Information Processing Systems 7},
pp.\ 609--616. Cambridge, MA: MIT Press.

[2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS: Exploring
  Realistic Neural Models with the GEneral NEural SImulation System.}  New York:
TELOS/Springer--Verlag.

[3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of learning and
recall at excitatory recurrent synapses and cholinergic modulation in rat
hippocampal region CA3. {\it Journal of Neuroscience} {\bf 15}(7):5249-5262.
